$\Pi_{2}^{P}$ vs PSpace Dichotomy for the Quantified Constraint Satisfaction Problem

The Quantified Constraint Satisfaction Problem is the problem of evaluating a sentence with both quantifiers, over relations from some constraint language, with conjunction as the only connective. We show that for any constraint language on a finite domain the Quantified Constraint Satisfaction Problem is either in $\Pi_{2}^{P}$, or PSpace-complete. Additionally, we build a constraint language on a 6-element domain such that the Quantified Constraint Satisfaction Problem over this language is $\Pi_{2}^{P}$-complete.

==> Definitions.tex <==



\noindent\rule[0.5ex]{\linewidth}{1pt}
\section{Definitions and notations}


% \textbf{Induced relations}
% For every $R$ and $m \in \{0,1,\dots,n\}$ we define 
% two relations. 
% \begin{align*}
% \mathcal W_R^{m}
% (y_0,\dots,y_m,x_1,\dots,x_m)
% =&
% \forall x\exists y_{m+1}\exists y_{m+2}\dots\exists y_{n} 
% R(y_0,\dots,y_n,x_1,\dots,x_m,x,x,\dots,x),\\
% \mathcal S_R^{m}
% (y_0,\dots,y_m,x_1,\dots,x_m)
% =&
% \forall x\exists y_{m+1}\forall x'
% \exists y_{m+2}\dots\exists y_{n} 
% R(y_0,\dots,y_n,x_1,\dots,x_m,x,x',\dots,x').
% \end{align*}

% We set by definition that 
% $\mathcal S_R^{n}=\mathcal W_R^{n}=R$
% and $\mathcal S_R^{n-1}=\mathcal W_R^{n-1}$.
% Additionally we define 
% $$\mathcal {\widetilde W}_R^{m}
% (y_0,\dots,y_m,x_1,\dots,x_m)
% =\bigwedge\limits_{i=0}^{m}
% \mathcal {W}_R^{m}
% (y_0,\dots,y_i,x_1,\dots,x_i)
% $$
% $$\mathcal {\widetilde S}_R^{m}
% (y_0,\dots,y_m,x_1,\dots,x_m)
% =
% \mathcal {S}_R^{m}
% (y_0,\dots,y_m,x_1,\dots,x_m)
% \wedge \bigwedge\limits_{i=0}^{m-1}
% \mathcal {W}_R^{m}
% (y_0,\dots,y_i,x_1,\dots,x_i)
% $$

% \textbf{Formulas.}
% For a formula $\Phi$ and 
% free variables 
% $x_1,\dots,x_{n}$ of this formula 
% by 
% $\Phi_{x_1,\dots,x_{n}}^{y_1,\dots,y_n}$ we denote 
% denote the formula obtained from $\Phi$ 
% by replacement each variable $x_{i}$ by $y_{i}$.


\textbf{Parameterised CSP Instances, relations, and constraints .}
For a given CSP instance $\mathcal I$ we call some variables of this instance parameters (usually it is $z_{1},\dots,z_{k}$).
Then we refer to this instance as 
$\prescript{z_1,\dots,z_k}{}{\mathcal I}$.
We say that the instance $\prescript{z_1,\dots,z_k}{}{\mathcal I}$ satisfies some property 
$P$ if it satisfies this property for every $z_{1},\dots,z_{|A|}\in A$.  


% \textbf{Induced CSP Instance.}
% Suppose 
% $\mathcal I$ is an instance of $\QCSP(\Gamma)$, that is 
% $\mathcal I = \exists y_0 \forall x_1 \exists y_1 \dots
% \forall x_{n} \exists y_{n} 
% \Phi$, 
% where $\Phi$ is a conjunction of relations 
% from $\Gamma$.
% For every $\mathcal I$
% we can write 
% an equivalent exponential size CSP instance over the same language with constants as follows. 
% If the sentence 
% $\mathcal I$ holds then there exist Skolem functions 
% $f_{0},\dots,f_{n}$
% defining a winning strategy for the existential 
% player. 
% That is, she can play 
% $y_{i} = f_{i}(x_1,\dots,x_{i})$.
% Since it is a winning strategy, if the UP plays 
% $(x_{1},x_2,\dots,x_{n})=(a_1,a_2,\dots,a_{n})$ and 
% the EP plays 
% $(y_0,y_1,\dots,y_{n})=(f_{0}(),f_{1}(a_1),f_{2}(a_1,a_2),\dots,f_{n}(a_1,\dots,a_{n}))$,
% then the obtained evaluation should satisfy 
% the quantifier-free part $\Phi$.
% We can introduce 
% an existential variable 
% $y_{i}^{a_1,\dots,a_i}$ 
% for every $a_{1},\dots,a_{i}\in A$, 
% which is just a value of 
% $f_{i}(a_1,\dots,a_{i})$.
% Then 
% $\mathcal I$ is equivalent 
% to 
% $\bigwedge\limits_{a_1,\dots,a_{n}\in A}
% \Phi_{x_1,\dots,x_{n},y_1,y_2,\dots,y_{n}}^{a_1,\dots,a_{n},y_{1}^{a_1},y_{2}^{a_{1},a_2},\dots,y_{n}^{a_1,\dots,a_{n}}}.$

% Since usually we do not have constants in our 
% constraint language $\Gamma$ we consider a parameterized 
% CSP instance.

% For a conjunctive formula 
% $\Phi$ or a relation $R$ put 
% $$\ExpCSP_{n}(R)=
% \bigwedge_{(a_1,\dots,a_n)}
% R(y_{1},y_{2}^{a_1},y_{3}^{a_1 a_2},\dots,
% y_{n}^{a_1 a_2 a_3\dots a_{n-1}},
% z_{a_1},z_{a_2},z_{a_3},\dots,z_{a_n})
% $$




%COMMENT. 
%Whenever I write 
%$\prescript{\zv}{\delta} R_{2}^{\alpha}$ is reflexive, I mean it is reflexive for any 
%$\zv$, $\delta$, and $\alpha$.

%Every relation has its domain

We cannot use $\forall$ as value. 
Thus we need a separate claim that 
if $R_{0}^{\alpha} = |A|!\cdot R^{\alpha}$ 
then $R_{0}^{\forall}$
is transitive. 


%Adjacent constraints

%Index of a variable

%$\Phi(x)$ for a CSP instance $\Phi$.

%$[n]$

%Domain is always $A$.

%path

%length of a path

%connected subinstance

%child

%$\Level(y)$ 

%level of a variable

%lowest variable
%parameterised reduction

%q-definable

%$R+B$

%transitive closure

%$R\circ S$.

%$R^{\infty}$

%$R^{\infty\infty}$


%We say that one parameterized reduction is smaller than another if....
In this subsection we prove that 
for any 1-consistent $\zv$ parameterized reduction 
$D^{(\top)}$ 
of a $\mathcal I\ExpCSP(\Phi)$.
there exists a 1-consistent reduction
$D^{(\bot)}$
such that 
$\prescript{\zv}{} D^{(\bot)}
\triangleleft \prescript{\zv}{} D^{(\top)}$
for every $\zv\in A^{|A|}$ 
$\prescript{\zv}{} D^{(\bot)}\neq
\prescript{\zv}{} D^{(\top)}$
for some $\zv\in A^{|A|}$.
%We call this reduction \emph{smaller}.

%$A$ is fixed, $n$ is fixed.



%witness of $\zigzag$.

%universal weakening

%stronger instance


%coverings

%tree-coverings



%trivial $\zv$-parameterized unary subuniverse

%$\triangleleft$ and $\trianglelefteq$

%$\triangleleft^{s}$ and $\trianglelefteq^{s}$


%nonempty\\transitive relation
